Compositional Generalization Across Distributional Shifts with Sparse Tree Operations

Neural networks continue to struggle with compositional generalization, and this issue is exacerbated by a lack of massive pre-training. One successful approach for developing neural systems which exhibit human-like compositional generalization is \textit{hybrid} neurosymbolic techniques. However, these techniques run into the core issues that plague symbolic approaches to AI: scalability and flexibility. The reason for this failure is that at their core, hybrid neurosymbolic models perform symbolic computation and relegate the scalable and flexible neural computation to parameterizing a symbolic system. We investigate a \textit{unified} neurosymbolic system where transformations in the network can be interpreted simultaneously as both symbolic and neural computation. We extend a unified neurosymbolic architecture called the Differentiable Tree Machine in two central ways. First, we significantly increase the model's efficiency through the use of sparse vector representations of symbolic structures. Second, we enable its application beyond the restricted set of tree2tree problems to the more general class of seq2seq problems. The improved model retains its prior generalization capabilities and, since there is a fully neural path through the network, avoids the pitfalls of other neurosymbolic techniques that elevate symbolic computation over neural computation.

==> sections/s2_workshop/abstract.tex <==
\begin{abstract}
Neural networks continue to struggle with compositional generalization, and this issue is exacerbated by a lack of massive pre-training. One successful approach for developing neural systems which exhibit human-like compositional generalization is \textit{hybrid} neurosymbolic techniques. However, these techniques run into the core issues that plague symbolic approaches to AI: scalability and flexibility. The reason for this failure is that at their core, hybrid neurosymbolic models perform symbolic computation and relegate the scalable and flexible neural computation to parameterizing a symbolic system. We investigate a \textit{unified} neurosymbolic system where transformations in the network can be interpreted simultaneously as both symbolic and neural computation. We extend a unified neurosymbolic architecture called the Differentiable Tree Machine in two central ways. First, we significantly increase the model’s efficiency through the use of sparse vector representations of symbolic structures. Second, we enable its application beyond the restricted set of tree2tree problems to the more general class of seq2seq problems. The improved model retains its prior generalization capabilities and, since there is a fully neural path through the network, avoids the pitfalls of other neurosymbolic techniques that elevate symbolic computation over neural computation.
\end{abstract}

==> sections/s2_workshop/conclusion.tex <==
\section{Conclusions} \label{sec:conclusion}
We introduced the Sparse Differentiable Tree Machine (\sdtm) and a novel schema for efficiently representing trees in vector space: \fullrepname (\abvrepname).
 While not perfect --- \sdtm struggles with MCD and Template shifts, as well as the extremely small GeoQuery dataset --- the model generalizes robustly across the \textit{widest variety} of distributional shifts. \sdtm is also uniquely capable of zero-shot lexical generalization, likely enabled by its factorization of content and structure. While these capacities for generalization are shared with the original \dtm, our instantiation is computationally efficient (representing a 75x reduction in parameters) and can be applied to seq2seq, seq2tree, and tree2tree tasks. Our work reaffirms the ability of neurosymbolic approaches to bridge the flexibility of connectionist models with the generalization of symbolic systems. We believe continued focus on efficient neurosymbolic implementations can lead to architectures with the kinds of robust generalization, scalability, and flexibility characteristic of human intelligence.

%We introduced \fullrepname (\abvrepname) and the Sparse Differentiable Tree Machine (\sdtm) to achieve robust compositional generalization across a variety of datasets and distributional shifts. \abvrepname is an efficient format for representing trees in vector space and operating over them in a structured manner. \sdtm is an extension of \dtm to improve efficiency by using \abvrepname. We introduced techniques to apply \sdtm to seq2seq tasks.



% \hal{I think we need one high-level causal claim to explain the performance of DTM. This could be (ordering is vaguely from best to worst)

%     a) The use of a unified approach - symbols in vector space - rather than symbolic, connectionist, or hybrid results robustness to the largest number of distributional shifts. This is introduced in the intro pdf line 56. This is the clear distinct thing between DTM and baselines
%     b) Separate Treatment of structure and content, respects the underlying compositionality of the data - affording greater generalisation performance. This is introduced starting at pdf line 47, 67, and again at line 126. A major issue with this is that grammar induction and symbolic approaches like NQG also have distinct notions of structure and content
%     c) The DTM has compositional representations and compositional operations designed for them. To get robust generalisation you need both representational and operational compositionality. This is discussed at pdf lines: 102. While this is probably the truest explanation and best scoped, we don't compare with a symbolic stack machine or something else with compositional operations and I feel like we want a core claim to reiterate how the model is different from baselines - which the 'unified' argumentation does better. We also haven't made much of it in the writing so far}


%\hal{I think we really need to move limitations out of section 6. Not a super nice to end on}
% Our method has several limitations. MCD and Template shifts remain difficult for \sdtm. GeoQuery remains a difficult task, and our model was unable to make progress. More significantly, our model is non-autoregressive. This makes it difficult to apply to tasks which benefit greatly from autoregression \citep{huang2022directed}. Future work should look into integrating the sequence-input \dtm as an encoder with an autoregressive decoder.

==> sections/s2_workshop/introduction.tex <==
\section{Introduction}

\begin{wrapfigure}{r}{0.425\linewidth}
    \centering
    \vspace{-6.2em}
    \includegraphics[width=\linewidth]{sections/images/tight_radar/radar_integrated_legend.png}
    %\vspace{-2.5em}
    \caption{Generalization ability of our approach (\sdtm) compared with baselines across various out-of-distribution shifts, averaged over different datasets. See \S \ref{sec:results}.}
    \label{fig:enter-label}
    \vspace{-1.5em}
\end{wrapfigure}

\textbf{Note: this is an abbreviated version simultaneously published at the NeurIPS 2024 main conference. Please see that version for the full details.} Deep learning models achieve remarkable performance across a broad range of natural language tasks \citep{vaswani2017attention}, despite having difficulty generalizing outside of their training data, struggling with new words \citep{Lake_2018_GeneralizationSystematicityCompositional}, known words in new contexts \citep{keysers2020measuring}, and novel syntactic structures, like longer sequences with greater recursive depth \citep{kim-linzen-2020-cogs, li_slog_2023}. Increasingly this problem is addressed through data augmentation, which tries to make it less likely a model will encounter something unlike what it sees during training --- reducing the degree by which it has to generalize \citep{andreas_good-enough_2020, devlin_bert_2019,  guo_sequence-level_2020}. However, even models trained on vast quantities of data struggle when evaluated on examples unlike those seen during training \citep{kim2022uncontrolled}.


This stands in contrast to how humans process language, which enables robust generalization \citep{pinker2003language}. By breaking novel sentences into known parts, we can readily interpret phrases and constructions that we have never encountered before (e.g. `At the airport I smiled myself an upgrade', \citep{goldberg_constructions_2006}). Why do models trained on orders of magnitude more language data than a human hears in 200 lifetimes \citep{Griffiths2020UnderstandingHI} still fail to acquire some of language's most essential properties?

Central to language's generalizability is compositional structure \citep{partee1995lexical} where contentful units, like words, fit together in a structure, like a syntactic tree. Many classical approaches in NLP and Machine Learning attempt to induce a grammar from data in the hope of leveraging the same kinds of generalization seen in natural language \citep[e.g.][]{ klein2002generative, kim2019compound, steedman1987combinatory}. However, structured representations are not first-order primitives in most neural networks \citep{Marcus2001-MARTAM-10, Smolensky_1988}. Despite theoretical appeal, the strictures of purely discrete symbolic approaches have made them difficult to apply to the breadth of tasks and domains where deep learning models have proven successful \citep{furrer2020compositional}. In contrast, purely connectionist models --- like Transformers \citep{vaswani2017attention} --- struggle with the kinds of sample efficiency and robust generalization ubiquitous to human learning. 

Neurosymbolic methods attempt to integrate neural and symbolic techniques to arrive at a system that is both compositional and flexible \citep{nslr,garcez2008neural,GARNELO201917, Smolensky_1988}. While some neurosymbolic architectures achieve impressive compositional generalization, they are often brittle due to the symbolic core of their computation \citep{shaw-etal-2021-compositional}. These methods are hybrid neurosymbolic systems, where the primary computation is symbolic, and the neural network serves to parameterize the symbolic space. We take a different approach, one where symbolic operations happen in vector space. In our system, neural and symbolic computations are \textbf{unified} into a single space; we multiply and add vector-embedded symbolic structures instead of multiplying and adding individual neurons. Related Work is discussed in Appendix \ref{sec:related}. %This technique is known as blending and superposition. % vector-embedded symbolic structures are blended together by superimposing them.

We introduce a new technique for representing trees in vector space called \fullrepname (\abvrepname). \abvrepname allows us to perform structural operations: transformations which change the structure of an object without changing the content. This is a crucial aspect of compositionality, where the structure and content can be transformed independently. We extend a previous system which operates over binary trees in vector space, the Differentiable Tree Machine (\dtm), to improve performance and applicability to a larger variety of tasks\footnote{Code and data available at publication.}. While \dtm processes vector-embedded binary trees as the primitive unit of computation, the order of operations and argument selection is governed by a Transformer. We present results showing that this unified approach retains many of the desirable properties of more brittle symbolic models with regards to generalization, while remaining flexible enough to work across a far wider set of tasks. 
%Additionally we lay out a framework for evaluating generalization ability. Averaging scores across different tasks based on which of six different kinds of distributional shift they require a model to generalize to. 
While fully neural architectures or hybrid neurosymbolic techniques excel at certain types of generalization, we find that \dtm, with its unified approach,  excels across the widest array of shifts.

%In what follows we introduce a novel approach to unifying these lines of work;  a model architecture whose representational schema and internal operations are explicitly compositional, taking binary trees as its representational primitive. However, the order of operations applied and in what combination is governed by a transformer. We present results showing that this hybrid approach retains many of the desirable properties of more brittle symbolic models, while remaining flexible enough to work across a far wider set of tasks.

The main contributions from this paper are:
\begin{itemize}
  \item \fullrepname (\abvrepname), a method for representing binary trees in vector space. (\S\ref{sec:sparse-tpr})
  \item Bit-Shift Operating --- systematic and parallelized tree operations for \abvrepname. (\S\ref{sec:diff-tree-ops})
  \item The introduction of Sparse Differentiable Tree Machine (\sdtm), architectural improvements to the \dtm to leverage \abvrepname and drastically reduce parameter and memory usage. (\S\ref{sec:dtm-modifications})
  \item Techniques to apply \dtm to seq2seq tasks by converting sequences into trees. (\S\ref{sec:seq2tree})
  \item Empirical comparisons between \sdtm and various baselines showing \sdtm's strong generalization across a wide variety of tasks. (\S\ref{sec:results})
  %\item Ablation experiments to support our architectural decisions. (\paul{TODO on section})
\end{itemize}


% \begin{itemize}
%     \item \textbf{DTM \emph{Merge}}  --- An instantiation of the Differentiable Tree Machine Architecture for seq2seq tasks
%     \item \textbf{75x reduction in parameter count} --- improvements to the \dtm that drastically reduce parameter and memory usage. (\ref{sec:dtm-modifications})
%     \item \textbf{Sparse Coordinate Trees} --- a method for representing binary trees as sparse tensors (\ref{sec:sparse-tpr})
%     \item \textbf{Bit-Shift Operating} --- fast, parallelised, operations for Sparse Coordinate Trees
%     \item Empirical results showing \textbf{DTM \emph{Merge's}} strong generalisation performance across a wide array of generalisation challenges
% \end{itemize}



%Cognitive Science and Linguistics suggest that compositionality is achieved through the use of structured representations and program-like induction. However, structured representations are not first-order primitives in neural networks. This leads to scenarios where neural networks fail to generalize out-of-distribution in ways that are easy for humans \citep{kim-linzen-2020-cogs, Lake_2018_GeneralizationSystematicityCompositional}. Despite this seeming lack of structured representations, neural networks are the most successful technology to date which can capture the flexibility of human intelligence.

% \paul{Notes I wrote down when asking Paul to describe why TPRs are explicitly compositional. I think working this into the introduction as a benefit of our approach (as well as DTM1 and others) compared to modern NNs is a good idea: Factor data into two parallel streams. One stream is about structure, the other is about content alone. The same content can be used structurally in many different ways, which is the compositionality. It maintains its internal identity, such that wherever it is put, it has the same representation.}








==> sections/s2_workshop/model.tex <==
\section{The Sparse Differentiable Tree Machine (\sdtm)}
\label{sec:dtm-modifications}

Our work extends the Differentiable Tree Machine (\dtm) introduced in \citet{Soulos_2023_DifferentiableTreeOperations} with the Sparse Differentiable Tree Machine (\sdtm). While similar to the original at a computational level, \sdtm represents a different implementation of these concepts that make it dramatically more parameter and memory efficient. We also introduce techniques to apply \sdtm to tasks with sequence input and output (seq2seq). 

\subsection{Overview} \label{sec:dtm_sparse}
\begin{wrapfigure}[8]{r}{0.35\linewidth}
    \centering
    \vspace{-4em}
    \includegraphics[width=\linewidth]{sections/images/dtm-shrink.pdf}
    \caption{A schematic of how the three core components of the \dtm (agent, interpreter, and memory) relate to each other. Adapted from \citet{Soulos_2023_DifferentiableTreeOperations}.}
    \label{fig:dtm}
\end{wrapfigure}

\sdtm uses our \fullrepname schema across its components. Like the original \dtm, our model is comprised of an agent, interpreter, and memory (illustrated in Figure \ref{fig:dtm}). The Interpreter performs Equation \ref{eq:output} by applying the bit-shifting tree operations from Section \ref{sec:diff-tree-ops} and weighting the result. The output from the interpreter is written to the next available memory slot, and the last memory slot is taken as the output.

The Agent is a Transformer encoder that takes an encoding of the memory as input and produces the inputs for Equation \ref{eq:output}: $\vec{w}$, $\vec{T}$, and $s$. Two special tokens, <OP> and <ROOT>, are fed into the Agent to represent $\vec{w}$ and $s$. Each time a tree is written to memory, a fixed-dimensional encoding of that tree is produced and fed as a new token to the agent (\S \ref{sec:mha}). The agent soft-selects tree arguments for the interpreter, $\vec{T}$, by performing a weighted sum over the trees in memory. Figure \ref{fig:agent} in the Appendix contains a detailed diagram showing the flow of information for one layer of \sdtm.

\subsection{Pooling by attention} \label{sec:mha}

Each tree in memory needs to have a fixed-dimensional encoding to feed into the agent regardless of how many nodes are filled. Commonly this is done via pooling, like taking the means of the elements in the tree, or a linear transformation in the case of the original \dtm. Instead, we use Pooling by Multi-headed Attention (PMA) \citep{pmlr-v97-lee19d}, which performs a weighted sum over the elements, where the weight is derived based on query-key attention.

Attention is permutation invariant, but it is important that our pooling considers tree position information. To enforce this, we convert the position indices to their binary vector representation $\vec{b}$. This leads to an asymmetrical vector with only positive values, so instead we represent left branches as $-1$ and keep right branches as $+1$. For example, position $5 \rightarrow [0,0,0,0,0,1,0,1] \rightarrow [0,0,0,0,0,1,-1,1]$. The input to our pooling function is the concatenation of this positional encoding $\vec{b}$ with the token embedding $\vec{x}$ at that position: $[\vec{x};\vec{b}]$. This method for integrating token and node position is similar to tree positional encoding from \citet{NEURIPS2019_6e091746}, except that we use concatenation and a linear transformation to mix the content and position information instead of addition.

Unlike standard self attention, we use a separate, single learnable parameter for our query vector $\vec{q} \in \mathbb{R}^{\text{num\_heads}\times\text{key\_dim}}$. We pass $[\vec{x};\vec{b}]$ through linear transformations to generate keys $\vec{k} \in \mathbb{R}^{\text{num\_heads}\times\text{key\_dim}}$ and values $\vec{v} \in \mathbb{R}^{\text{num\_heads}\times\text{value\_dim}}$. The result of this computation is always $z \in \mathbb{R}^{\text{num\_heads}\times\text{value\_dim}}$ given that $\vec{q}$ is fixed and does not depend on the input. The rest of the computation is identical to a Transformer with pre-layer normalization \citep{xiong2020layer}.

\subsection{Tree Pruning} \label{sec:pruning}
While \fullrepname mean that trees with fewer filled nodes take up less memory, the way our model blends operations results in trees becoming dense.
%Our sparse tree representation works well when the trees themselves are sparse.
The interpreter returns a blend of all three operations at each step, including the \cons operation which increases the size of the representation by combining two trees. In practice even as the entropy of the blending distribution drops, the probability of any operation never becomes fully 0. This means that over many steps, trees start to become dense due to repeated use of \cons. In order to keep our trees sparse, we use pruning: only keeping the top-$k$ nodes as measured by magnitude. $k$ is a hyper-parameter that can be set along with the batch size depending on available memory. 

\subsection{Lexical Regularization} \label{sec:lex-reg}
To aid lexical generalization, we add noise to our token embeddings. Before feeding an embedded batch into the model, we sample from a multi-variate standard normal for each position in each tree, adding the noise to the embeddings as a form of regularization \citep{bishop-noise}. Ablation results showing the importance of this regularization are available in Appendix \ref{sec:lex-reg-ablation}. %Particularly on low-resource tasks, with a small input vocabulary --- like SCAN --- this regularisation proves essential. We believe this kind of regularisation forces the model to use a larger subspace to represent each token, which makes token representations more resilient to the kinds of novel contextualisations posed by lexical generalisation challenges. This approach to lexical regularisation can be easily applied to most models, and may improve generalisation in low-resource settings. 

%We find this regularization essential for lexical generalization as shown in \paul{TODO! Probably a table in the appendix}. We sample the noise from a standard normal distribution.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{sections/images/root nodes and laud shrink.pdf}
    \caption{Left: The memory state is initialized as a sequence of trees where only the root node contains a token. Right: An output sequence is embedded in a tree using the left-aligned uniform-depth (LAUD) scheme. <NT> and <EOB> are special tokens not in the original output sequence.}
    \label{fig:root-and-laud}
\end{figure}

\subsection{Handling Sequential Inputs and Outputs}\label{sec:seq2tree}
\paragraph{seq2tree} The original \dtm can only be applied to tasks where a tree structure is known for both inputs and outputs. Here we provide an extension to allow \dtm to process sequence inputs. To do this we treat each input token as a tree with only the root node occupied by the token embedding. We then initialize the tree memory with $N$ trees, one for each token in the input sequence. Figure \ref{fig:root-and-laud} left depicts the initial memory state for a sequence. The agent's attention mechanism is permutation-invariant, so in order to distinguish between two sequences which contain the same tokens but in different orders, we apply random sinusoidal positional encodings to the first $N$ tokens passed to the agent \citep{li2023representations, ruoss-etal-2023-randomized}. Random positional encodings sample a set of increasing integers from left-to-right instead of assigning a fixed position to each token. The purpose of \leftcommand and \rightcommand is to extract subtrees. Since in our seq2tree setting the input sequence is processed in a completely bottom-up manner, we restrict the agent and interpreter to only have a single operation: \cons. Use of a single operation to construct new trees from subtrees aligns the \dtm theoretically with the Minimalist Program \citep{10.7551/mitpress/9780262527347.001.0001}, which addresses natural language's compositionality in terms of a single operation: merge.
\paragraph{seq2seq} To handle sequence inputs and outputs we convert the output sequence to a tree. One method to convert the output sequence into a tree is to use a parser. Alternatively, when a parser is not available, we can embed a sequence as the \textbf{l}eft-\textbf{a}ligned leaves at \textbf{u}niform \textbf{d}epth (LAUD). Figure \ref{fig:root-and-laud} right shows how an output sequence can be embedded using LAUD. Since all of the non-terminal nodes are the same, we can hardcode the root argument to \cons. We insert a special token <EOB> to signify the end of a branch, similar to an <EOS> token.



==> sections/s2_workshop/results.tex <==
\section{Results} \label{sec:results}

We consider models that are trained from scratch on the datasets they're evaluated on; while the compositional capabilities of large pre-trained models are under active debate \citep{kim2022uncontrolled}, we are interested in the compositional abilities of the underlying architecture --- rather than those that may result from a pre-training objective.
%believe that there is a benefit in developing models that learn from exposure to a single task. \paul{Other reasons to consider only models exposed to a task are for building human-like intelligence which isn't exposed to mass data as well as computing costs.} 
We compare \dtm to two fully neural models, a standard Transformer \citep{vaswani2017attention} as well as a relative universal Transformer (RU-Transformer) which was previously shown to improve systematic generalization on a variety of tasks \citep{csordas-etal-2021-devil}. We also compare our model to a hybrid neurosymbolic system, NQG \citep{shaw-etal-2021-compositional, Sun_2023_ReplicationStudyCompositional}, a model which uses a neural network to learn a quasi-synchronous context-free grammar \citep{smith-eisner-2006-quasi}. NQG was introduced alongside NQG-T5, which is a modular system that uses NQG when the grammar produces an answer and falls back to a fine-tuned large language model T5 \citep{t5}. As mentioned at the beginning of this section, we only compare to NQG in this paper since we want to evaluate models that have not undergone significant pre-training.\footnote{NQG uses pre-trained BERT embeddings \citep{devlin_bert_2019}; it is unknown how much this pre-training helps the method.} Details related to data preprocessing (\S\ref{sec:data-preprocessing}), model training (\S\ref{sec:dtm-training}, \S\ref{sec:baseline-training}), and compute resources (\S\ref{sec:compute-resources}) are available in the Appendix.

For each task, we test whether models generalize to samples drawn from various data distributions. Independent and identically distributed (\textbf{IID}) samples are drawn from a distribution shared with training data. We evaluate several out-of-distribution (OOD) shifts. \textbf{One-shot} lexical samples, while drawn from the same distribution as the training data, contain a word that was only seen in a single training sample. Similarly, \textbf{Zero-shot} lexical samples are those where the model is not exposed to a word at all during training. \textbf{Structural/length} generalization tests whether models can generalize to longer sequences (length) or nodes not encountered during training (structural). \textbf{Template} generalization withholds an abstract n-gram sequence during training, and then each test sample fits the template. Finally, maximum compound divergence (\textbf{MCD}) generates train and test sets with identical uni-gram distributions but maximally divergent n-grams frequencies \citep{keysers2020measuring}. Although models are often tested on a single type of generalization, we believe evaluating a model across a broad array of distributional shifts is essential for characterizing the robustness of its generalization performance.

\begin{table}
  \caption{\textbf{Active$\leftrightarrow$Logical accuracy.} Results are the best performance over five runs. The test sets are divided into IID, and OOD sets 0-shot lexical and structural. Parameter and memory usage is shown for the original \dtm with TPRs and our proposed sparse \dtm with and without pruning. Our modifications reduce the parameter count by almost two orders of magnitude. $^\ast$NQG was trained on a seq2seq version without parantheses because it was not able to learn the tree2tree training set.}
  \label{tab:activelogical}
  \centering
  \begin{tabular}{llllll}
    \toprule
    Model & \multicolumn{3}{c}{Split}         \\
    \cmidrule(r){2-4}
    & IID & 0-Shot Lexical & Structural \\
    \cmidrule(r){1-4}
    Transformer    & $1.0$ & $0.0$ & $0.0$ \\
    RU-Transformer & $1.0$ & $0.0$ & $.12$ \\
    NQG$^\ast$            & $.45$ & $0.0$ & $0.0$ \\
    \midrule
    & & & & Parameters & Memory (GB) \\
    \midrule
    Original \dtm  & $1.0$ & $1.0$ & $1.0$ & 72M & 12.3  \\ 
    \sdtm  & $1.0$ & $1.0$ & $1.0$ & 1M & 9.7     \\
    \sdtm (pruned k=1024) & $1.0$ & $1.0$ & $.95$ & 1M & 1.8 \\
    \bottomrule
\end{tabular}
\end{table}

\subsection{Performance Regression (Active$\leftrightarrow$Logical)} \label{sec:previous-dtm-comparison}
Active$\leftrightarrow$Logical is a tree2tree task containing input and output trees in active voice and logical forms \citep{Soulos_2023_DifferentiableTreeOperations}. Transforming a tree in active voice to its logical form simulates semantic parsing, and transforming a logical form tree to active voice simulates natural language generation. For this dataset, there are three test sets: IID, 0-shot lexical, and structural. In addition to the baselines listed in the previous section, we also compare our modified \sdtm to the original \dtm to see the changes in parameter count and memory. The results are show in Table \ref{tab:activelogical}.

The various \dtm models and Transformers all perform perfectly on the IID test set. NQG struggles to learn the Active$\leftrightarrow$Logical task, an example of the brittleness of hybrid neurosymbolic systems. Only the \dtm variants succeed on the OOD test sets. As anticipated, the RU-Transformer performs better than the standard Transformer with regards to structural generalization.

Comparing the original \dtm to \sdtm without pruning, we see a 70x reduction in parameter count from pooling by attention, as well as a 20\% reduction in memory usage from fewer parameters and \abvrepname. We are able to gain even further memory savings due to the pruning method. The final two rows show that the pruning method has no impact on lexical generalization and a minor impact on structural generalization, while reducing memory usage by 5x. The results from this experiment confirm that \sdtm is capable of matching \dtm performance on a previous baseline. Next we turn to tasks where the original \dtm could not be used.

\subsection{Scalability (FOR2LAM)}
FOR2LAM is a tree2tree program translation task to translate an abstract syntax tree (AST) in an imperative language FOR to an AST in a functional language LAM \citep{NEURIPS2018_d759175d}. This makes FOR2LAM a good dataset to test the scalability of \sdtm to more complex samples. We augment the FOR2LAM dataset with a 0-shot lexical test set. During training, only two variable names appear: `x' and `y'. For the 0-shot test, we replace all occurrences of x in the test set with a new token `z'. We are unable to test \dtm on FOR2LAM because a batch of 1 does not fit into memory due to the depth of the trees.

Results on FOR2LAM are shown on the left side of Table \ref{tab:for2lam_geoquery}. NQG suffers with scale (see \ref{sec:baseline-training}), and we were unable to include results for it on FOR2LAM due to training and evaluation exceeding 7 days. All other models do well on the in-distribution test set, but only \dtm is able to achieve substantive accuracy on the 0-shot lexical test. \dtm's performance is impressive given work on data augmentation has shown the difficulty of few-shot generalization is inversely proportional to vocabulary size \citep{patel2022revisiting}, with smaller vocabulary tasks being more challenging. This 0-shot challenge is from 2 variables (x, y) to 3 (x, y, z), making it difficult enough that both transformer variants score 0.03\%.
ta
\subsection{Seq2Tree (GeoQuery)}


\begin{table}
\centering
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{\textbf{FOR2LAM}} & \multicolumn{4}{c}{\textbf{GeoQuery}} \\
\cmidrule(r){2-3} \cmidrule(l){4-7}
Model & IID & 0-shot lexical & IID & Length & Template & TMCD \\
\midrule
Transformer & 1.0 & .03 & .88 & .26 & .79 & .40 \\
RU-Transformer & 1.0 & .03 & .87 & .25 & .77 & .37 \\
NQG$^\dag$ & -- & -- & .76 & .37/.26$^\ast$ & .62 & .41 \\
\midrule
\sdtm & 1.0 & .61 & .73 & .18 & .20 & .35 \\
\bottomrule
\end{tabular}
\caption{\textbf{Accuracies on FOR2LAM and GeoQuery.} Results are the best performance over five runs. $^\dag$Results taken from \citet{shaw-etal-2021-compositional}. $^\ast$We report the results from a replication study of NQG where the result on the Length split differed substantially from the original result \citep{Sun_2023_ReplicationStudyCompositional}.}
\label{tab:for2lam_geoquery}
\end{table}

GeoQuery is a natural language to SQL dataset \citep{zelle1996learning} where a model needs to map a question stated in natural language to a correctly formatted SQL query, including parentheses to mark functions and arguments. We use the parentheses and function argument relationship as the tree structure for our output. In this format, GeoQuery is a seq2tree task, and we follow the description from Section \ref{sec:seq2tree}.  We use the same preprocessing and data as \citet{shaw-etal-2021-compositional}. The TMCD split for GeoQuery \citep{shaw-etal-2021-compositional} extends MCD to natural language datasets instead of synthetic languages. GeoQuery is a very small dataset, with a training set containing between 440 and 600 samples, depending on the split. We are unable to test \dtm on GeoQuery because a batch size of 1 does not fit into memory.

Results for GeoQuery are shown on the right side of Table \ref{tab:for2lam_geoquery}. This is the most difficult task that we test because of the small training set, and the natural language input is not draw from a synthetic grammar. Given this, a potential symbolic solution to this task might be quite complex. We find that both NQG and \dtm perform worse than the two Transformer variants on the IID test set. This also holds true for the Template split, where Transformers outperform the neurosymbolic models. On the Length and TMCD splits, all of the baselines achieve roughly the same performance while \dtm performs slightly worse --- the degree of variation in the input space and small training set appear to make it difficult for \sdtm to find a compositional solution. 
%\paul{Can we justify this performance a bit?}

\subsection{Seq2Seq (SCAN)}
SCAN is a synthetic seq2seq task with training and test variations to examine OOD generalization \citep{Lake_2018_GeneralizationSystematicityCompositional}. To process seq2seq samples, we follow the description in Section \ref{sec:seq2tree}. We compare two methods for embedding the output sequence into a tree by writing a parser for SCAN's output and comparing this to the left-aligned uniform-depth trees (LAUD). In addition to the standard test splits from SCAN, we introduce a 0-shot lexical test set as well.

\begin{table}
  \caption{\textbf{SCAN accuracy.} Results are the best performance over five runs. MCD scores are calculated as the average of the three MCD splits. $^\dag$Results from \citet{shaw-etal-2021-compositional}. $^\ast$Results from \citet{Sun_2023_ReplicationStudyCompositional}.}
  \label{tab:scan}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Model & \multicolumn{6}{c}{Split}         \\
    \cmidrule(r){2-7}
    & IID & 1-shot lexical & 0-shot lexical & Length & Template & MCD \\
    \midrule
    Transformer & 1.0 & .08 & 0.0 & .07 & 1.0 & .02 \\
    RU-Transformer & 1.0 & .11 & 0.0 & .19 & 1.0 & .01 \\
    NQG$^\dag$ & 1.0$^\ast$ & 1.0 & 0.0 & 1.0 & 0.0$^\ast$ & 1.0     \\
    \midrule
    \sdtm (parse trees)     & 1.0   & .99 & .99 & .75 & .95 & .03  \\
    \sdtm (LAUD trees) & 1.0 & .87 & .98 & .06 & .98 & 0.0 \\
    \bottomrule
\end{tabular}
\end{table}

All models perform well on the IID test set, showing that they have learned the training distribution well. Transformer variants perform poorly on lexical, length, and MCD splits. 
%The RU-Transformer does better than the standard Transformer on the length split, but \citet{csordas-etal-2021-devil} showed that the RU-Transformer needs an easier length shift to increase its performance more.
The Transformers and \sdtm perform well on the Template split while NQG completely fails. Along with the results from GeoQuery, which showed weak \sdtm performance on the Template split and strong performance from both Transformers, it seems that the Transformer architecture is robust under template shifts between training and testing. \sdtm is the only model to perform well on the 0-shot lexical test set, whereas NQG is the only model able to perform well on the MCD test set. The two \sdtm rows compare models trained with output trees from a parser or LAUD encoding. The main performance difference is on the Length split, where the structurally relevant information in the parse trees is necessary for \sdtm to perform well. It is not necessary to have structured input for the model to perform well on length generalization as long as the output is structured.



==> sections/s2_workshop/sparse_tpr.tex <==
\section{Differentiable Tree Operations Over \fullrepname}
Representing trees in vector space enables us to perform differentiable structural operations on them. 
%However, before we can define the  operations, we need a representational format for embedding trees in vector space. 
\citet{Soulos_2023_DifferentiableTreeOperations} used Tensor Product Representations (TPRs) \citep{Smolensky1990TensorPV} for this purpose. TPRs use the tensor (or outer) product to represent trees in vector space (\S\ref{sec:appendix-sparse-tprs}). Use of an outer product leads to a representation dimensionality that is multiplicative with both the embedding dimensionality and the number of possible tree nodes. Additionally, the number of nodes is itself an exponential function of the supported depth. This makes TPRs difficult to use in practice, given available memory is quickly exceeded as tree depth increases.


In this section, we introduce \fullrepname (\abvrepname), a new schema for representing trees in vector space. We then define a library of parallelized tree operations and how to perform these operations on \abvrepname.




\label{sec:sparse-tpr}
Like TPRs, we want an encoding for trees that factorizes the representation into subspaces for \emph{structure} and \emph{content} respectively. This approach to representational spaces differs from models like an RNN and Transformer, which represent structure and content jointly in an unfactorized manner.
%many of today's popular neural networks which learn representations in an unfactorized manner. 
By separating the structure and content subspaces a priori, we can operate over these two spaces independently. This decision is motivated by the fact that distinct treatment of these spaces is an essential aspect of compositionality.


\begin{wrapfigure}[22]{o}{0.33\linewidth}
    \centering
    \vspace{-2em}
    \includegraphics[width=\linewidth]{sections/images/figure 2 vertical.pdf}
    \caption{An example representation using \fullrepname (\abvrepname). The values are N-dimensional vectors, and the tree positional indices are integer representations of positions in the tree. The absent child nodes of "The" (indices 4 and 6) are skipped with \abvrepname.}
    \label{fig:sparse-tpr}
\end{wrapfigure}


We derive our tree representation scheme from the sparse coordinate list (COO) format. COO stores tensor data in tuples of (indices [integers], values [any format], size [integers]). The indices are N-dimensional to simulate a tensor of arbitrary shape (e.g. including dimensions such as batch or length). When an index is not indicated in indices, it is assumed that the corresponding value is 0.

We give structural meaning to COO representations by defining one dimension of indices as the tree position occupied by a value vector. Our tree addressing scheme is based on Gorn addresses \citep{gorn+1967+77+115}: to get the tree position from an index, convert the index to binary and read from right to left. A left-branch is indicated by a $0$ and a right branch by a $1$. To distinguish between leading $0$s and left-branches (e.g. $010$ vs $10$), we start our addressing scheme at $1$ instead of $0$. This indicates that all $0$s to the left of the most-significant $1$ are unfilled and not left-branches. 
Figure \ref{fig:sparse-tpr} shows an example encoding of a tree with this approach. \abvrepname can be viewed as a TPR with certain constraints, and Section \ref{sec:appendix-sparse-tprs} defines this equivalence and describes the memory savings.

Section \ref{sec:previous-dtm-comparison} discusses the performance, memory, and parameter comparison between \dtm models which use TPRs and \abvrepname.

\subsection{Differentiable Tree Operations} \label{sec:diff-tree-ops}

To operate on the trees defined in the previous section, we need a set of functions. We use a small library of only three: left-child (\leftcommand), right-child (\rightcommand), and \textbf{cons}truct (\cons) a new tree from a left and right subtree.\footnote{In LISP and expert systems literature, \leftcommand is referred to as \car, and \rightcommand is referred to as \cdr.} Although these three functions are simple, along with the control operations of conditional branching and equality-checking, these five functions are Turing complete \citep{mccarthy1960recursive}.

In addition to saving memory, \abvrepname also provides a more efficient method for performing differentiable tree operations. The operations defined in \citet{Soulos_2023_DifferentiableTreeOperations} require precomputing, storing, and applying linear transformations for \leftcommand, \rightcommand, and \cons. Since our values and tree positional indices are kept separate, we can compute the results of \leftcommand, \rightcommand, and \cons dramatically more efficiently using indexing, bit-shifts, and addition.



Figure \ref{fig:sparse-operations} shows how we can perform \leftcommand directly on \abvrepname. \leftcommand is performed by indexing the even indices (i.e. those with a 0 in the least significant bit, which targets all of the nodes left of the root) and their corresponding values, then performing a right bit-shift on the indices. \rightcommand is symmetrical, except that we index for the odd positional indices and ignore position 1 in order to remove the previous root node. \cons is performed by left bit-shifting the positional indices from the left- and right-subtree arguments, then adding 1 to the newly shifted indices for the right argument. A new value $s$ can be provided for the root node.



Our network also needs to learn a \textit{program} over multiple operations differentiably. This involves the aforementioned structured operations, as well as differentiable selection of which operation to perform and on which trees. We take weighted sums over the three operations \leftcommand, \rightcommand, and \cons, as well as over potential trees. Specific details are discussed in the next section. The result of our weighted sum is coalesced, which removes duplicate positional indices by summing together all of the values that share a specific index. 
Formally, define the trees over which to perform \leftcommand \ $T_{L}$, \rightcommand \ $T_{R}$, and \cons \ $T_{CL}$ \& $T_{CR}$; $\vec{T}=[T_{L};T_{R};T_{CL};T_{CR}]$. We  also take a new value $s \in \mathbb{R}^{d}$ to be inserted ($\otimes$) at the new root node of the \cons operation, and a vector of operation weights $\vec{w} = (w_L,  w_R, w_C)$ which sum to 1.

\begin{equation} \label{eq:output}
O(\vec{w}, \vec{T}, s) = w_L \leftcommand(T_{L}) + w_R \rightcommand(T_{R}) + w_C ( \cons(T_{CL}, T_{CR}) +  s \otimes r_{1})
\end{equation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sections/images/left and right.pdf}
    \caption{Left: Performing \leftcommand (orange) and \rightcommand (blue). Right: visualizing the \leftcommand transformation which results in DP being placed at the root. Tree positional indices of $0$ and their corresponding values are discarded.}
    \label{fig:sparse-operations}
\end{figure}

==> sections/submission/abstract.tex <==
\begin{abstract}
Neural networks continue to struggle with compositional generalization, and this issue is exacerbated by a lack of massive pre-training. One successful approach for developing neural systems which exhibit human-like compositional generalization is \textit{hybrid} neurosymbolic techniques. However, these techniques run into the core issues that plague symbolic approaches to AI: scalability and flexibility. The reason for this failure is that at their core, hybrid neurosymbolic models perform symbolic computation and relegate the scalable and flexible neural computation to parameterizing a symbolic system. We investigate a \textit{unified} neurosymbolic system where transformations in the network can be interpreted simultaneously as both symbolic and neural computation. We extend a unified neurosymbolic architecture called the Differentiable Tree Machine in two central ways. First, we significantly increase the model’s efficiency through the use of sparse vector representations of symbolic structures. Second, we enable its application beyond the restricted set of tree2tree problems to the more general class of seq2seq problems. The improved model retains its prior generalization capabilities and, since there is a fully neural path through the network, avoids the pitfalls of other neurosymbolic techniques that elevate symbolic computation over neural computation.
\end{abstract}

==> sections/submission/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: At the end of the introduction, we outline the primary contributions of our paper along with the associated section where that content is available.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We address limitations of our approach in Section \ref{sec:conclusion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide mathematical descriptions of our model, but we do not introduce any proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main content outlines our model and empirical setup. In Appendix \ref{sec:dtm-training} we provide details for training our model, and in Appendix \ref{sec:baseline-training} we outline details for training the baselines. Additionally, we plan to make our code and data open source at the time of publication to facilitate reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we plan to make our code and data open source at the time of publication to facilitate reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The data splits are discussed extensively in Section \ref{sec:results}. In Appendix \ref{sec:dtm-training} we provide details for training our model, and in Appendix \ref{sec:baseline-training} we outline details for training the baselines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: for our results, we report the best run across five random initializations. As discussed in Appendix \ref{sec:dtm-training}, neurosymbolic technique can have high variance, and this method of reporting results is common.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In Appendix \ref{sec:compute-resources} we discuss the compute resources needed to run our experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This research is upstream of any concrete applications. While there is always a risk of scientific research, we do not believe this work contains risks beyond general scientific research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This research is upstream of any concrete applications. While there is always a risk of scientific research, we do not believe this work contains risks beyond general scientific research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This research is upstream of any concrete applications. While there is always a risk of scientific research, we do not believe this work contains risks beyond general scientific research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cited the papers that introduce the models and datasets that we use. Most of the models and datasets we used are publicly available. Appendix \ref{sec:licenses} contains additional information with regards to the licenses of each asset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we plan to make our code and data open source at the time of publication to facilitate reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve crowdsourcing nor human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve crowdsourcing nor human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sections/submission/conclusion.tex <==
\section{Conclusions} \label{sec:conclusion}
We introduced the Sparse Differentiable Tree Machine (\sdtm) and a novel schema for efficiently representing trees in vector space: \fullrepname (\abvrepname).
Unlike the fully neural and hybrid neurosymbolic baselines presented here, \sdtm takes a unified approach whereby symbolic operations occur in vector space. While not perfect --- \sdtm struggles with MCD and Template shifts, as well as the extremely small GeoQuery dataset --- the model generalizes robustly across the \textit{widest variety} of distributional shifts. \sdtm is also uniquely capable of zero-shot lexical generalization, likely enabled by its factorization of content and structure.

While these capacities for generalization are shared with the original \dtm, our instantiation is computationally efficient (representing a 75x reduction in parameters) and can be applied to seq2seq, seq2tree, and tree2tree tasks. Our work reaffirms the ability of neurosymbolic approaches to bridge the flexibility of connectionist models with the generalization of symbolic systems. We believe continued focus on efficient neurosymbolic implementations can lead to architectures with the kinds of robust generalization, scalability, and flexibility characteristic of human intelligence.

%We introduced \fullrepname (\abvrepname) and the Sparse Differentiable Tree Machine (\sdtm) to achieve robust compositional generalization across a variety of datasets and distributional shifts. \abvrepname is an efficient format for representing trees in vector space and operating over them in a structured manner. \sdtm is an extension of \dtm to improve efficiency by using \abvrepname. We introduced techniques to apply \sdtm to seq2seq tasks.



% \hal{I think we need one high-level causal claim to explain the performance of DTM. This could be (ordering is vaguely from best to worst)

%     a) The use of a unified approach - symbols in vector space - rather than symbolic, connectionist, or hybrid results robustness to the largest number of distributional shifts. This is introduced in the intro pdf line 56. This is the clear distinct thing between DTM and baselines
%     b) Separate Treatment of structure and content, respects the underlying compositionality of the data - affording greater generalisation performance. This is introduced starting at pdf line 47, 67, and again at line 126. A major issue with this is that grammar induction and symbolic approaches like NQG also have distinct notions of structure and content
%     c) The DTM has compositional representations and compositional operations designed for them. To get robust generalisation you need both representational and operational compositionality. This is discussed at pdf lines: 102. While this is probably the truest explanation and best scoped, we don't compare with a symbolic stack machine or something else with compositional operations and I feel like we want a core claim to reiterate how the model is different from baselines - which the 'unified' argumentation does better. We also haven't made much of it in the writing so far}


%\hal{I think we really need to move limitations out of section 6. Not a super nice to end on}
% Our method has several limitations. MCD and Template shifts remain difficult for \sdtm. GeoQuery remains a difficult task, and our model was unable to make progress. More significantly, our model is non-autoregressive. This makes it difficult to apply to tasks which benefit greatly from autoregression \citep{huang2022directed}. Future work should look into integrating the sequence-input \dtm as an encoder with an autoregressive decoder.

==> sections/submission/introduction.tex <==
\section{Introduction}

\begin{wrapfigure}{r}{0.425\linewidth}
    \centering
    \vspace{-1.2em}
    \includegraphics[width=\linewidth]{sections/images/tight_radar/radar_integrated_legend.png}
    %\vspace{-2.5em}
    \caption{Generalization ability of our approach (\sdtm) compared with baselines across various out-of-distribution shifts, averaged over different datasets. See \S \ref{sec:results}.}
    \label{fig:enter-label}
    \vspace{-1.5em}
\end{wrapfigure}

Deep learning models achieve remarkable performance across a broad range of natural language tasks \citep{vaswani2017attention}, despite having difficulty generalizing outside of their training data, struggling with new words \citep{Lake_2018_GeneralizationSystematicityCompositional}, known words in new contexts \citep{keysers2020measuring}, and novel syntactic structures, like longer sequences with greater recursive depth \citep{kim-linzen-2020-cogs, li_slog_2023}. Increasingly this problem is addressed through data augmentation, which tries to make it less likely a model will encounter something unlike what it sees during training --- reducing the degree by which it has to generalize \citep{andreas_good-enough_2020, devlin_bert_2019,  guo_sequence-level_2020}. However, even models trained on vast quantities of data struggle when evaluated on examples unlike those seen during training \citep{kim2022uncontrolled}.


This stands in contrast to how humans process language, which enables robust generalization \citep{pinker2003language}. By breaking novel sentences into known parts, we can readily interpret phrases and constructions that we have never encountered before (e.g. `At the airport I smiled myself an upgrade', \citep{goldberg_constructions_2006}). Why do models trained on orders of magnitude more language data than a human hears in 200 lifetimes \citep{Griffiths2020UnderstandingHI} still fail to acquire some of language's most essential properties?

Central to language's generalizability is compositional structure \citep{partee1995lexical} where contentful units, like words, fit together in a structure, like a syntactic tree. Many classical approaches in NLP and Machine Learning attempt to induce a grammar from data in the hope of leveraging the same kinds of generalization seen in natural language \citep[e.g.][]{ klein2002generative, kim2019compound, steedman1987combinatory}. However, structured representations are not first-order primitives in most neural networks \citep{Marcus2001-MARTAM-10, Smolensky_1988}. Despite theoretical appeal, the strictures of purely discrete symbolic approaches have made them difficult to apply to the breadth of tasks and domains where deep learning models have proven successful \citep{furrer2020compositional}. In contrast, purely connectionist models --- like Transformers \citep{vaswani2017attention} --- struggle with the kinds of sample efficiency and robust generalization ubiquitous to human learning. 

Neurosymbolic methods attempt to integrate neural and symbolic techniques to arrive at a system that is both compositional and flexible \citep{nslr,garcez2008neural,GARNELO201917, Smolensky_1988}. While some neurosymbolic architectures achieve impressive compositional generalization, they are often brittle due to the symbolic core of their computation \citep{shaw-etal-2021-compositional}. These methods are hybrid neurosymbolic systems, where the primary computation is symbolic, and the neural network serves to parameterize the symbolic space. We take a different approach, one where symbolic operations happen in vector space. In our system, neural and symbolic computations are \textbf{unified} into a single space; we multiply and add vector-embedded symbolic structures instead of multiplying and adding individual neurons. %This technique is known as blending and superposition. % vector-embedded symbolic structures are blended together by superimposing them.

We introduce a new technique for representing trees in vector space called \fullrepname (\abvrepname). \abvrepname allows us to perform structural operations: transformations which change the structure of an object without changing the content. This is a crucial aspect of compositionality, where the structure and content can be transformed independently. We extend a previous system which operates over binary trees in vector space, the Differentiable Tree Machine (\dtm), to improve performance and applicability to a larger variety of tasks\footnote{Code and data available at publication.}. While \dtm processes vector-embedded binary trees as the primitive unit of computation, the order of operations and argument selection is governed by a Transformer. We present results showing that this unified approach retains many of the desirable properties of more brittle symbolic models with regards to generalization, while remaining flexible enough to work across a far wider set of tasks. 
%Additionally we lay out a framework for evaluating generalization ability. Averaging scores across different tasks based on which of six different kinds of distributional shift they require a model to generalize to. 
While fully neural architectures or hybrid neurosymbolic techniques excel at certain types of generalization, we find that \dtm, with its unified approach,  excels across the widest array of shifts.

%In what follows we introduce a novel approach to unifying these lines of work;  a model architecture whose representational schema and internal operations are explicitly compositional, taking binary trees as its representational primitive. However, the order of operations applied and in what combination is governed by a transformer. We present results showing that this hybrid approach retains many of the desirable properties of more brittle symbolic models, while remaining flexible enough to work across a far wider set of tasks.

The main contributions from this paper are:
\begin{itemize}
  \item \fullrepname (\abvrepname), a method for representing binary trees in vector space as sparse tensors. (\S\ref{sec:sparse-tpr})
  \item Bit-Shift Operating --- systematic and parallelized tree operations for \abvrepname. (\S\ref{sec:diff-tree-ops})
  \item The introduction of Sparse Differentiable Tree Machine (\sdtm), architectural improvements to the \dtm to leverage \abvrepname and drastically reduce parameter and memory usage. (\S\ref{sec:dtm-modifications})
  \item Techniques to apply \dtm to seq2seq tasks by converting sequences into trees. (\S\ref{sec:seq2tree})
  \item Empirical comparisons between \sdtm and various baselines showing \sdtm's strong generalization across a wide variety of tasks. (\S\ref{sec:results})
  %\item Ablation experiments to support our architectural decisions. (\paul{TODO on section})
\end{itemize}


% \begin{itemize}
%     \item \textbf{DTM \emph{Merge}}  --- An instantiation of the Differentiable Tree Machine Architecture for seq2seq tasks
%     \item \textbf{75x reduction in parameter count} --- improvements to the \dtm that drastically reduce parameter and memory usage. (\ref{sec:dtm-modifications})
%     \item \textbf{Sparse Coordinate Trees} --- a method for representing binary trees as sparse tensors (\ref{sec:sparse-tpr})
%     \item \textbf{Bit-Shift Operating} --- fast, parallelised, operations for Sparse Coordinate Trees
%     \item Empirical results showing \textbf{DTM \emph{Merge's}} strong generalisation performance across a wide array of generalisation challenges
% \end{itemize}



%Cognitive Science and Linguistics suggest that compositionality is achieved through the use of structured representations and program-like induction. However, structured representations are not first-order primitives in neural networks. This leads to scenarios where neural networks fail to generalize out-of-distribution in ways that are easy for humans \citep{kim-linzen-2020-cogs, Lake_2018_GeneralizationSystematicityCompositional}. Despite this seeming lack of structured representations, neural networks are the most successful technology to date which can capture the flexibility of human intelligence.

% \paul{Notes I wrote down when asking Paul to describe why TPRs are explicitly compositional. I think working this into the introduction as a benefit of our approach (as well as DTM1 and others) compared to modern NNs is a good idea: Factor data into two parallel streams. One stream is about structure, the other is about content alone. The same content can be used structurally in many different ways, which is the compositionality. It maintains its internal identity, such that wherever it is put, it has the same representation.}








==> sections/submission/model.tex <==
\section{The Sparse Differentiable Tree Machine (\sdtm)}
\label{sec:dtm-modifications}

Our work extends the Differentiable Tree Machine (\dtm) introduced in \citet{Soulos_2023_DifferentiableTreeOperations} with the Sparse Differentiable Tree Machine (\sdtm). While similar to the original at a computational level, \sdtm represents a different implementation of these concepts that make it dramatically more parameter and memory efficient. We also introduce techniques to apply \sdtm to tasks with sequence input and output (seq2seq). 

\subsection{Overview} \label{sec:dtm_sparse}
\begin{wrapfigure}{r}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{sections/images/dtm.pdf}
    \caption{A schematic of how the three core components of the \dtm (agent, interpreter, and memory) relate to each other. Adapted from \citet{Soulos_2023_DifferentiableTreeOperations}.}
    \label{fig:dtm}
\end{wrapfigure}

\sdtm uses our \fullrepname schema across its components. Like the original \dtm, our model is comprised of an agent, interpreter, and memory (illustrated in Figure \ref{fig:dtm}). The Interpreter performs Equation \ref{eq:output} by applying the bit-shifting tree operations from Section \ref{sec:diff-tree-ops} and weighting the result. The output from the interpreter is written to the next available memory slot, and the last memory slot is taken as the output.

The Agent is a Transformer encoder that takes an encoding of the memory as input and produces the inputs for Equation \ref{eq:output}: $\vec{w}$, $\vec{T}$, and $s$. Two special tokens, <OP> and <ROOT>, are fed into the Agent to represent $\vec{w}$ and $s$. Each time a tree is written to memory, a fixed-dimensional encoding of that tree is produced and fed as a new token to the agent (\S \ref{sec:mha}). The agent soft-selects tree arguments for the interpreter, $\vec{T}$, by performing a weighted sum over the trees in memory. Figure \ref{fig:agent} in the Appendix contains a detailed diagram showing the flow of information for one layer of \sdtm.

\subsection{Pooling by attention} \label{sec:mha}

Each tree in memory needs to have a fixed-dimensional encoding to feed into the agent regardless of how many nodes are filled. Commonly this is done via pooling, like taking the means of the elements in the tree, or a linear transformation in the case of the original \dtm. Instead, we use Pooling by Multi-headed Attention (PMA) \citep{pmlr-v97-lee19d}, which performs a weighted sum over the elements, where the weight is derived based on query-key attention.

Attention is permutation invariant, but it is important that our pooling considers tree position information. To enforce this, we convert the position indices to their binary vector representation $\vec{b}$. This leads to an asymmetrical vector with only positive values, so instead we represent left branches as $-1$ and keep right branches as $+1$. For example, position $5 \rightarrow [0,0,0,0,0,1,0,1] \rightarrow [0,0,0,0,0,1,-1,1]$. The input to our pooling function is the concatenation of this positional encoding $\vec{b}$ with the token embedding $\vec{x}$ at that position: $[\vec{x};\vec{b}]$. This method for integrating token and node position is similar to tree positional encoding from \citet{NEURIPS2019_6e091746}, except that we use concatenation and a linear transformation to mix the content and position information instead of addition.

Unlike standard self attention, we use a separate, single learnable parameter for our query vector $\vec{q} \in \mathbb{R}^{\text{num\_heads}\times\text{key\_dim}}$. We pass $[\vec{x};\vec{b}]$ through linear transformations to generate keys $\vec{k} \in \mathbb{R}^{\text{num\_heads}\times\text{key\_dim}}$ and values $\vec{v} \in \mathbb{R}^{\text{num\_heads}\times\text{value\_dim}}$. The result of this computation is always $z \in \mathbb{R}^{\text{num\_heads}\times\text{value\_dim}}$ given that $\vec{q}$ is fixed and does not depend on the input. The rest of the computation is identical to a Transformer with pre-layer normalization \citep{xiong2020layer}.

\subsection{Tree Pruning} \label{sec:pruning}
While \fullrepname mean that trees with fewer filled nodes take up less memory, the way our model blends operations results in trees becoming dense.
%Our sparse tree representation works well when the trees themselves are sparse.
The interpreter returns a blend of all three operations at each step, including the \cons operation which increases the size of the representation by combining two trees. In practice even as the entropy of the blending distribution drops, the probability of any operation never becomes fully 0. This means that over many steps, trees start to become dense due to repeated use of \cons. In order to keep our trees sparse, we use pruning: only keeping the top-$k$ nodes as measured by magnitude. $k$ is a hyper-parameter that can be set along with the batch size depending on available memory. 

\subsection{Lexical Regularization} \label{sec:lex-reg}
To aid lexical generalization, we add noise to our token embeddings. Before feeding an embedded batch into the model, we sample from a multi-variate standard normal for each position in each tree, adding the noise to the embeddings as a form of regularization \citep{bishop-noise}. Ablation results showing the importance of this regularization are available in Appendix \ref{sec:lex-reg-ablation}. %Particularly on low-resource tasks, with a small input vocabulary --- like SCAN --- this regularisation proves essential. We believe this kind of regularisation forces the model to use a larger subspace to represent each token, which makes token representations more resilient to the kinds of novel contextualisations posed by lexical generalisation challenges. This approach to lexical regularisation can be easily applied to most models, and may improve generalisation in low-resource settings. 

%We find this regularization essential for lexical generalization as shown in \paul{TODO! Probably a table in the appendix}. We sample the noise from a standard normal distribution.

\subsection{Handling Sequential Inputs and Outputs}\label{sec:seq2tree}
\paragraph{seq2tree} The original \dtm can only be applied to tasks where a tree structure is known for both inputs and outputs. Here we provide an extension to allow \dtm to process sequence inputs. To do this we treat each input token as a tree with only the root node occupied by the token embedding. We then initialize the tree memory with $N$ trees, one for each token in the input sequence. Figure \ref{fig:root-and-laud} left depicts the initial memory state for a sequence. The agent's attention mechanism is permutation-invariant, so in order to distinguish between two sequences which contain the same tokens but in different orders, we apply random sinusoidal positional encodings to the first $N$ tokens passed to the agent \citep{li2023representations, ruoss-etal-2023-randomized}. Random positional encodings sample a set of increasing integers from left-to-right instead of assigning a fixed position to each token. The purpose of \leftcommand and \rightcommand is to extract subtrees. Since in our seq2tree setting the input sequence is processed in a completely bottom-up manner, we restrict the agent and interpreter to only have a single operation: \cons. Use of a single operation to construct new trees from subtrees aligns the \dtm theoretically with the Minimalist Program \citep{10.7551/mitpress/9780262527347.001.0001}, which addresses natural language's compositionality in terms of a single operation: merge.
\paragraph{seq2seq} To handle sequence inputs and outputs we convert the output sequence to a tree. One method to convert the output sequence into a tree is to use a parser. Alternatively, when a parser is not available, we can embed a sequence as the \textbf{l}eft-\textbf{a}ligned leaves at \textbf{u}niform \textbf{d}epth (LAUD). Figure \ref{fig:root-and-laud} right shows how an output sequence can be embedded using LAUD. Since all of the non-terminal nodes are the same, we can hardcode the root argument to \cons. We insert a special token <EOB> to signify the end of a branch, similar to an <EOS> token.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{sections/images/root nodes and laud.pdf}
    \caption{Left: The memory state is initialized as a sequence of trees where only the root node contains a token. Right: An output sequence is embedded in a tree using the left-aligned uniform-depth (LAUD) scheme. <NT> and <EOB> are special tokens not in the original output sequence.}
    \label{fig:root-and-laud}
\end{figure}

==> sections/submission/related.tex <==
\section{Related Work}
Work leveraging the generalizability of tree structures has a long history across Computer Science, Linguistics, and Cognitive Science \citep{chomsky_aspects_1965,mccarthy1960recursive, sakai1961syntax,  Smolensky1990TensorPV, steedman1987combinatory}. Much of classical NLP aims to extract structured representations from text like constituency or dependency parses \citep[for overview:][]{cuetos2013parsing, lopez2008statistical}. More recent work has shown the representations learned by sequence-to-sequence models without structural supervision can recover constituency, dependency, and part of speech information from latent representations in machine translation and language models \citep{belinkov2019analysis, blevins2018deep}. While those analyses show structural information is encoded, they stop short of showing that the representations themselves are tree-structured. Analyses inspired by Tensor Product Representations \citep{mccoy2018rnns, soulos2019discovering} and chart parsing \citep{murty2022characterizing} give an account of how representations become somewhat tree-structured over the course of training.% In particular correlating out-of-distribution performance with prevalence of structure.

Despite the apparent emergence of semi-structured representations in transformers and LSTMs, these architectures still appear to struggle with the kinds of structural generalization that come easily to humans \citep{Lake_2018_GeneralizationSystematicityCompositional, kim_cogs_2020, keysers2020measuring}. A variety of approaches try to tackle this problem through meta-learning \citep{lake2019compositional, conklin2021meta}, data augmentation \citep{andreas_good-enough_2020}, or decomposing the task into separate parts \citep{ russin2019compositional, lindemann2023compositional}. The Relative-Universal Transformer \citep{csordas-etal-2021-devil} combines relative positional embeddings with a recurrent component, in an effort to emphasize local structures while allowing for unbounded computation.

%While in some cases effective these methods often have in-built costs in terms of training time, memory use, or domain generality - sometimes only working a small subset of tasks.



Explicitly tree structured network architectures have been introduced for RNNs \citep{socher-etal-2012-semantic}, LSTMs \citep{tai2015improved, dong2016language}, and Transformers \citep{wang2019tree, shiv2019novel}. However, these variants often do not outperform their unstructured counterpart on out-of-distribution challenges \citep{Soulos_2023_DifferentiableTreeOperations}. This may be because generalization requires both structured representations and operations that respect that structure. A separate line of work considers neural architectures that are used to parameterize components of a symbolic system \cite{kim2019compound, chen2020compositional} or that leverage explicit stack operations \citep{dusell2024stack, grefenstette2015learning, joulin2015inferring, yogatama2018memory}. NQG from \citet{shaw-etal-2021-compositional} combines the outputs from neural and symbolic models by inducing a grammar, but deferring to T5 \citep{t5} when that grammar fails. However the grammar's induction method has polynomial complexity with both dataset size and sequence length, which limits its application to larger tasks.

%Work that has neural components but a symbolic core: NQG (Compositional generalization and natural language variation: our model can handle both), Kim's NQCFG, The Nye work on program synthesis for SCAN, Neural symbolic stack machines.

%Meta-learning/auxiliary task and data augmentation (only works for lexical) approaches to compositionality.

%Work interpreting trees in neural networks (hewitt, murty, Tom's thesis, etc)

%Trees in neural networks (TreeRNN, TreeLSTM, Tree Transformer) can represent tree information, but don't have a way to modify trees with symbolic operations. TreeRNNs compress the tree, which makes it difficult to reconstruct the tree and perform systematic operations. For instance, we would want the encoding for a large tree passed through a left child operation to match the encoding of the left subchild built from the bottom up.

%Superposition Stacks function similar to our new sparse implicit method (cite joulin, gref, yogatama, dusell).

%Most similar to our work is that of \citet{Soulos_2023_DifferentiableTreeOperations}. In that work, trees are also represented in vector space and differentiable tree operations are derived.  However, they only apply their technique on Tree2Tree tasks, and their technique has limitations which make it computationally expensive. We show how to extend their approach to solve Seq2Tree and Seq2Seq tasks, and we also propose theoretical and applied changes to drastically improve the memory efficiency of their technique.

Vector Symbolic Architectures (VSAs) implement symbolic algorithms while leveraging high dimensional spaces \citep{plate, gayler2003vsa_jackendoff, kanerva2009hyperdimensional, kleyko2022}. VSAs are similar to uniform neurosymbolic approaches, although VSAs commonly lack a learning component. Our work extends that of \citet{Soulos_2023_DifferentiableTreeOperations} which can be viewed as integrating Deep Learning and VSAs. They introduce the Differentiable Tree Machine for Tree-to-Tree transduction. Here we instantiate a sparse Sequence-to-Sequence version with far fewer parameters and improved memory efficiency.

%The representation schema we use that enables this efficiency is similar to that of superposition stacks \cite{dusell2021learning}, though designed for tree-structures.

==> sections/submission/results.tex <==
\section{Results} \label{sec:results}

\subsection{Baselines}
We consider models that are trained from scratch on the datasets they're evaluated on; while the compositional capabilities of large pre-trained models are under active debate \citep{kim2022uncontrolled}, we are interested in the compositional abilities of the underlying architecture --- rather than those that may result from a pre-training objective.
%believe that there is a benefit in developing models that learn from exposure to a single task. \paul{Other reasons to consider only models exposed to a task are for building human-like intelligence which isn't exposed to mass data as well as computing costs.} 
We compare \dtm to two fully neural models, a standard Transformer \citep{vaswani2017attention} as well as a relative universal Transformer (RU-Transformer) which was previously shown to improve systematic generalization on a variety of tasks \citep{csordas-etal-2021-devil}. We also compare our model to a hybrid neurosymbolic system, NQG \citep{shaw-etal-2021-compositional, Sun_2023_ReplicationStudyCompositional}, a model which uses a neural network to learn a quasi-synchronous context-free grammar \citep{smith-eisner-2006-quasi}. NQG was introduced alongside NQG-T5, which is a modular system that uses NQG when the grammar produces an answer and falls back to a fine-tuned large language model T5 \citep{t5}. As mentioned at the beginning of this section, we only compare to NQG in this paper since we want to evaluate models that have not undergone significant pre-training.\footnote{NQG uses pre-trained BERT embeddings \citep{devlin_bert_2019}; it is unknown how much this pre-training helps the method.} Details related to data preprocessing (\S\ref{sec:data-preprocessing}), model training (\S\ref{sec:dtm-training}, \S\ref{sec:baseline-training}), and compute resources (\S\ref{sec:compute-resources}) are available in the Appendix.

For each task, we test whether models generalize to samples drawn from various data distributions. Independent and identically distributed (\textbf{IID}) samples are drawn from a distribution shared with training data. We evaluate several out-of-distribution (OOD) shifts. \textbf{One-shot} lexical samples, while drawn from the same distribution as the training data, contain a word that was only seen in a single training sample. Similarly, \textbf{Zero-shot} lexical samples are those where the model is not exposed to a word at all during training. \textbf{Structural/length} generalization tests whether models can generalize to longer sequences (length) or nodes not encountered during training (structural). \textbf{Template} generalization withholds an abstract n-gram sequence during training, and then each test sample fits the template. Finally, maximum compound divergence (\textbf{MCD}) generates train and test sets with identical uni-gram distributions but maximally divergent n-grams frequencies \citep{keysers2020measuring}. Although models are often tested on a single type of generalization, we believe evaluating a model across a broad array of distributional shifts is essential for characterizing the robustness of its generalization performance.

\begin{table}
  \caption{\textbf{Active$\leftrightarrow$Logical accuracy.} Results are the best performance over five runs. The test sets are divided into IID, and OOD sets 0-shot lexical and structural. Parameter and memory usage is shown for the original \dtm with TPRs and our proposed sparse \dtm with and without pruning. Our modifications reduce the parameter count by almost two orders of magnitude. $^\ast$NQG was trained on a seq2seq version without parantheses because it was not able to learn the tree2tree training set.}
  \label{tab:activelogical}
  \centering
  \begin{tabular}{llllll}
    \toprule
    Model & \multicolumn{3}{c}{Split}         \\
    \cmidrule(r){2-4}
    & IID & 0-Shot Lexical & Structural \\
    \cmidrule(r){1-4}
    Transformer    & $1.0$ & $0.0$ & $0.0$ \\
    RU-Transformer & $1.0$ & $0.0$ & $.12$ \\
    NQG$^\ast$            & $.45$ & $0.0$ & $0.0$ \\
    \midrule
    & & & & Parameters & Memory (GB) \\
    \midrule
    Original \dtm  & $1.0$ & $1.0$ & $1.0$ & 72M & 12.3  \\ 
    \sdtm  & $1.0$ & $1.0$ & $1.0$ & 1M & 9.7     \\
    \sdtm (pruned k=1024) & $1.0$ & $1.0$ & $.95$ & 1M & 1.8 \\
    \bottomrule
\end{tabular}
\end{table}

\subsection{Active$\leftrightarrow$Logical} \label{sec:previous-dtm-comparison}
Active$\leftrightarrow$Logical is a tree2tree task containing input and output trees in active voice and logical forms \citep{Soulos_2023_DifferentiableTreeOperations}. Transforming a tree in active voice to its logical form simulates semantic parsing, and transforming a logical form tree to active voice simulates natural language generation. For this dataset, there are three test sets: IID, 0-shot lexical, and structural. In addition to the baselines listed in the previous section, we also compare our modified \sdtm to the original \dtm to see the changes in parameter count and memory. The results are show in Table \ref{tab:activelogical}.

The various \dtm models and Transformers all perform perfectly on the IID test set. NQG struggles to learn the Active$\leftrightarrow$Logical task, an example of the brittleness of hybrid neurosymbolic systems. Only the \dtm variants succeed on the OOD test sets. As anticipated, the RU-Transformer performs better than the standard Transformer with regards to structural generalization.

Comparing the original \dtm to \sdtm without pruning, we see a 70x reduction in parameter count from pooling by attention, as well as a 20\% reduction in memory usage from fewer parameters and \abvrepname. We are able to gain even further memory savings due to the pruning method. The final two rows show that the pruning method has no impact on lexical generalization and a minor impact on structural generalization, while reducing memory usage by 5x.

\subsection{FOR2LAM}
FOR2LAM is a tree2tree program translation task to translate an abstract syntax tree (AST) in an imperative language (FOR) to an AST in a functional language (LAM) \citep{NEURIPS2018_d759175d}. We augment the FOR2LAM dataset with a 0-shot lexical test set. During training, only two variable names appear: `x' and `y'. For the 0-shot test, we replace all occurrences of x in the test set with a new token `z'.



\begin{wraptable}{l}{0.48\linewidth}
  \caption{\textbf{FOR2LAM accuracy.} Results are the best performance over five runs.}
  \label{tab:for2lam}
  \centering
  \begin{tabular}{lll}
    \toprule
    Model & \multicolumn{2}{c}{Split}         \\
    \cmidrule(r){2-3}
    & IID & 0-shot lexical \\
    \midrule
    Transformer & 1.0 & .03 \\
    RU-Transformer & 1.0 & .03 \\
    \midrule
    \sdtm     & 1.0     & .61   \\
    \bottomrule
\end{tabular}
\end{wraptable}

Results on FOR2LAM are shown in Table \ref{tab:for2lam}. NQG suffers with scale (see \ref{sec:baseline-training}), and we were unable to include results for it on FOR2LAM due to training and evaluation exceeding 7 days. All other models do well on the in-distribution test set, but only \dtm is able to achieve substantive accuracy on the 0-shot lexical test. \dtm's performance is impressive given work on data augmentation has shown the difficulty of few-shot generalization is inversely proportional to vocabulary size \citep{patel2022revisiting}, with smaller vocabulary tasks being more challenging. This 0-shot challenge is from 2 variables (x, y) to 3 (x, y, z), making it difficult enough that both transformer variants score 0.03\%.

\subsection{GeoQuery}

GeoQuery is a natural language to SQL dataset \citep{zelle1996learning} where a model needs to map a question stated in natural language to a correctly formatted SQL query, including parentheses to mark functions and arguments. We use the parentheses and function argument relationship as the tree structure for our output. In this format, GeoQuery is a seq2tree task, and we follow the description from Section \ref{sec:seq2tree}.  We use the same preprocessing and data as \citet{shaw-etal-2021-compositional}. The TMCD split for GeoQuery \citep{shaw-etal-2021-compositional} extends MCD to natural language datasets instead of synthetic languages. GeoQuery is a very small dataset, with a training set containing between 440 and 600 samples, depending on the split.

\begin{table}[b]
  \caption{\textbf{GeoQuery accuracy.} Results are the best performance over five runs. $^\dag$Results taken from \citet{shaw-etal-2021-compositional}.  $^\ast$We report the results from a replication study of NQG where the result on the Length split differed substantially from the original result \citep{Sun_2023_ReplicationStudyCompositional}.}
  \label{tab:geoquery}
  \centering
  \begin{tabular}{lllll}
    \toprule
    Model & \multicolumn{4}{c}{Split}         \\
    \cmidrule(r){2-5}
    & IID & Length & Template & TMCD \\
    \midrule
    Transformer & .88 & .26 &	.79 & 	.40 \\
    RU-Transformer & .87 &	.25 & .77 &	.37 \\
    NQG$^\dag$ & .76 & .37/.26$^\ast$ & .62 & .41     \\
    \midrule
    \sdtm     & .73 & .18 & .20 & .35  \\
    \bottomrule
\end{tabular}
\end{table}

Results for GeoQuery are shown in Table \ref{tab:geoquery}. This is the most difficult task that we test because of the small training set, and the natural language input is not draw from a synthetic grammar. Given this, a potential symbolic solution to this task might be quite complex. We find that both NQG and \dtm perform worse than the two Transformer variants on the IID test set. This also holds true for the Template split, where Transformers outperform the neurosymbolic models. On the Length and TMCD splits, all of the baselines achieve roughly the same performance while \dtm performs slightly worse --- the degree of variation in the input space and small training set appear to make it difficult for \sdtm to find a compositional solution. 
%\paul{Can we justify this performance a bit?}

\subsection{SCAN}
SCAN is a synthetic seq2seq task with training and test variations to examine out-of-distribution generalization \citep{Lake_2018_GeneralizationSystematicityCompositional}. To process seq2seq samples, we follow the description in Section \ref{sec:seq2tree}. We compare two methods to embedding the output sequence into a tree by writing a parser for SCAN's output and comparing this to the left-aligned uniform-depth trees (LAUD). In addition to the standard test splits from SCAN, we introduce a 0-shot lexical test set as well.

\begin{table}
  \caption{\textbf{SCAN accuracy.} Results are the best performance over five runs. MCD scores are calculated as the average of the three MCD splits. $^\dag$Results from \citet{shaw-etal-2021-compositional}. $^\ast$Results from \citet{Sun_2023_ReplicationStudyCompositional}.}
  \label{tab:scan}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Model & \multicolumn{6}{c}{Split}         \\
    \cmidrule(r){2-7}
    & IID & 1-shot lexical & 0-shot lexical & Length & Template & MCD \\
    \midrule
    Transformer & 1.0 & .08 & 0.0 & .07 & 1.0 & .02 \\
    RU-Transformer & 1.0 & .11 & 0.0 & .19 & 1.0 & .01 \\
    NQG$^\dag$ & 1.0$^\ast$ & 1.0 & 0.0 & 1.0 & 0.0$^\ast$ & 1.0     \\
    \midrule
    \sdtm (parse trees)     & 1.0   & .99 & .99 & .75 & .95 & .03  \\
    \sdtm (LAUD trees) & 1.0 & .87 & .98 & .06 & .98 & 0.0 \\
    \bottomrule
\end{tabular}
\end{table}

All models perform well on the IID test set, showing that they have learned the training distribution well. Transformer variants perform poorly on lexical, length, and MCD splits. 
%The RU-Transformer does better than the standard Transformer on the length split, but \citet{csordas-etal-2021-devil} showed that the RU-Transformer needs an easier length shift to increase its performance more.
The Transformers and \sdtm perform well on the Template split while NQG completely fails. Along with the results from GeoQuery, which showed weak \sdtm performance on the Template split and strong performance from both Transformers, it seems that the Transformer architecture is robust under template shifts between training and testing. \sdtm is the only model to perform well on the 0-shot lexical test set, whereas NQG is the only model able to perform well on the MCD test set. The two \sdtm rows compare models trained with output trees from a parser or LAUD encoding. The main performance difference is on the Length split, where the structurally relevant information in the parse trees is necessary for \sdtm to perform well. It is not necessary to have structured input for the model to perform well on length generalization as long as the output is structured.



==> sections/submission/sparse_tpr.tex <==
\section{Differentiable Tree Operations Over \fullrepname}
Representing trees in vector space enables us to perform differentiable structural operations on them. 
%However, before we can define the  operations, we need a representational format for embedding trees in vector space. 
\citet{Soulos_2023_DifferentiableTreeOperations} used Tensor Product Representations (TPRs) \citep{Smolensky1990TensorPV} for this purpose. TPRs use the tensor (or outer) product to represent trees in vector space (\S\ref{sec:appendix-sparse-tprs}). Use of an outer product leads to a representation dimensionality that is multiplicative with both the embedding dimensionality and the number of possible tree nodes. Additionally, the number of nodes is itself an exponential function of the supported depth. This makes TPRs difficult to use in practice, given available memory is quickly exceeded as tree depth increases.

In this section, we introduce \fullrepname (\abvrepname), a new schema for representing trees in vector space. We then define a library of parallelized tree operations and how to perform these operations on \abvrepname.

\subsection{\fullrepname (\abvrepname)} 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{sections/images/sparse coordinate tree.pdf}
    \caption{An example representation using \fullrepname (\abvrepname). The values are N-dimensional vectors, and the tree positional indices are integer representations of positions in the tree. The absent child nodes of "The" (indices 4 and 6) are skipped with \abvrepname.}
    \label{fig:sparse-tpr}
\end{figure}

\label{sec:sparse-tpr}
Like TPRs, we want an encoding for trees that factorizes the representation into subspaces for \emph{structure} and \emph{content} respectively. This approach to representational spaces differs from models like an RNN and Transformer, which represent structure and content jointly in an unfactorized manner.
%many of today's popular neural networks which learn representations in an unfactorized manner. 
By separating the structure and content subspaces a priori, we can operate over these two spaces independently. This decision is motivated by the fact that distinct treatment of these spaces is an essential aspect of compositionality.

We derive our tree representation scheme from the sparse coordinate list (COO) format. COO stores tensor data in tuples of (indices [integers], values [any format], size [integers]). The indices are N-dimensional to simulate a tensor of arbitrary shape (e.g. including dimensions such as batch or length). When an index is not indicated in indices, it is assumed that the corresponding value is 0.

We give structural meaning to COO representations by defining one dimension of indices as the tree position occupied by a value vector. Our tree addressing scheme is based on Gorn addresses \citep{gorn+1967+77+115}: to get the tree position from an index, convert the index to binary and read from right to left. A left-branch is indicated by a $0$ and a right branch by a $1$. To distinguish between leading $0$s and left-branches (e.g. $010$ vs $10$), we start our addressing scheme at $1$ instead of $0$. This indicates that all $0$s to the left of the most-significant $1$ are unfilled and not left-branches. 
Figure \ref{fig:sparse-tpr} shows an example encoding of a tree with this approach. \abvrepname can be viewed as a TPR with certain constraints, and Section \ref{sec:appendix-sparse-tprs} defines this equivalence and formally describes the memory savings.

Section \ref{sec:previous-dtm-comparison} discusses the performance, memory, and parameter comparison between \dtm models which use standard TPRs and \abvrepname.

\subsection{Differentiable Tree Operations} \label{sec:diff-tree-ops}

To operate on the trees defined in the previous section, we need a set of functions. We use a small library of only three: left-child (\leftcommand), right-child (\rightcommand), and \textbf{cons}truct (\cons) a new tree from a left and right subtree.\footnote{In LISP and expert systems literature, \leftcommand is referred to as \car, and \rightcommand is referred to as \cdr.} Although these three functions are simple, along with the control operations of conditional branching and equality-checking, these five functions are Turing complete \citep{mccarthy1960recursive}.

In addition to saving memory, \abvrepname also provides a more efficient method for performing differentiable tree operations. The operations defined in \citet{Soulos_2023_DifferentiableTreeOperations} require precomputing, storing, and applying linear transformations for \leftcommand, \rightcommand, and \cons. Since our values and tree positional indices are kept separate, we can compute the results of \leftcommand, \rightcommand, and \cons dramatically more efficiently using indexing, bit-shifts, and addition.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{sections/images/left and right.pdf}
    \caption{Left: Performing \leftcommand (orange) and \rightcommand (blue). Right: visualizing the \leftcommand transformation which results in DP being placed at the root. Tree positional indices of $0$ and their corresponding values are discarded.}
    \label{fig:sparse-operations}
\end{figure}

Figure \ref{fig:sparse-operations} shows how we can perform \leftcommand directly on \abvrepname. \leftcommand is performed by indexing the even indices (i.e. those with a 0 in the least significant bit, which targets all of the nodes left of the root) and their corresponding values, then performing a right bit-shift on the indices. \rightcommand is symmetrical, except that we index for the odd positional indices and ignore position 1 in order to remove the previous root node. \cons is performed by left bit-shifting the positional indices from the left- and right-subtree arguments, then adding 1 to the newly shifted indices for the right argument. A new value $s$ can be provided for the root node.


Our network also needs to learn a \textit{program} over multiple operations differentiably. This involves the aforementioned structured operations, as well as differentiable selection of which operation to perform and on which trees. We take weighted sums over the three operations \leftcommand, \rightcommand, and \cons, as well as over potential trees. Specific details are discussed in the next section. The result of our weighted sum is coalesced, which removes duplicate positional indices by summing together all of the values that share a specific index. 
Formally, define the trees over which to perform \leftcommand \ $T_{L}$, \rightcommand \ $T_{R}$, and \cons \ $T_{CL}$ \& $T_{CR}$; $\vec{T}=[T_{L};T_{R};T_{CL};T_{CR}]$. We  also take a new value $s \in \mathbb{R}^{d}$ to be inserted ($\otimes$) at the new root node of the \cons operation, and a vector of operation weights $\vec{w} = (w_L,  w_R, w_C)$ which sum to 1.

\begin{equation} \label{eq:output}
O(\vec{w}, \vec{T}, s) = w_L \leftcommand(T_{L}) + w_R \rightcommand(T_{R}) + w_C ( \cons(T_{CL}, T_{CR}) +  s \otimes r_{1})
\end{equation}
